Constrained Reinforcement Learning using Distributional Representation for Trustworthy Quadrotor UAV Tracking Control

Simultaneously accurate and reliable tracking control for quadrotors in complex dynamic environments is challenging. As aerodynamics derived from drag forces and moment variations are chaotic and difficult to precisely identify, most current quadrotor tracking systems treat them as simple `disturbances' in conventional control approaches. We propose a novel, interpretable trajectory tracker integrating a Distributional Reinforcement Learning disturbance estimator for unknown aerodynamic effects with a Stochastic Model Predictive Controller (SMPC). The proposed estimator `Constrained Distributional Reinforced disturbance estimator' (ConsDRED) accurately identifies uncertainties between true and estimated values of aerodynamic effects. Simplified Affine Disturbance Feedback is used for control parameterization to guarantee convexity, which we then integrate with a SMPC. We theoretically guarantee that ConsDRED achieves at least an optimal global convergence rate and a certain sublinear rate if constraints are violated with an error decreases as the width and the layer of neural network increase. To demonstrate practicality, we show convergent training in simulation and real-world experiments, and empirically verify that ConsDRED is less sensitive to hyperparameter settings compared with canonical constrained RL approaches. We demonstrate our system improves accumulative tracking errors by at least 70% compared with the recent art. Importantly, the proposed framework, ConsDRED-SMPC, balances the tradeoff between pursuing high performance and obeying conservative constraints for practical implementations.

==> NtP.tex <==
This work is motivated by challenges in training Reinforcement Learning (RL) for autonomous navigation in unmanned aerial vehicles, but its implications extend to other high-criticality applications in healthcare and financial services. The implementation of RL algorithm policies may exhibit various deficiencies, including (\textit{i}) opaque or unstable training due to the blackbox nature of deep neural networks, (\textit{ii}) difficulty in reproducing RL outcomes, and (\textit{iii}) heightened costs associated with robustness investigation, e.g., hyperparameter tuning and generalization. We present a novel `Constrained Distributional Reinforced disturbance estimator' (ConsDRED) to identify uncertainties arising from aerodynamic disturbances in agile flight. The proposed algorithm demonstrates at least an optimal convergence rate for both global optimization and constraint violations. Theoretical guarantees offered by this approach can make training convergence processes more transparent and provide a degree of confidence in the expected convergence outcomes in real-world applications, thereby addressing, to a considerable extent, the deficiencies related to (\textit{i}) and (\textit{ii}). Our robustness investigation empirically demonstrates that ConsDRED is significantly less sensitive to hyperparameter settings compared to traditional Constrained RL approaches. The experiments further showcase the generalization capability of ConsDRED through the introduction of new and previously unseen external forces in real-world scenarios.
It is noteworthy that while ConsDRED strikes a reasonable balance between performance and interpretability, there remains a trade-off with conservative decision making. Hence, we must strike a balance between the desired degree of interpretability and the acceptable level of scalability in RL algorithms. Another limitation is the computational complexity, where we sample at 16 Hz for disturbance estimation owing to limited onboard computational resources. This may be improved in future by implementation on dedicated hardware.
